On Minimum Trace Factor Analysis -- An Old Song Sung to a New Tune

Dimensionality reduction methods, such as principal component analysis (PCA) and factor analysis, are central to many problems in data science. There are, however, serious and well-understood challenges to finding robust low dimensional approximations for data with significant heteroskedastic noise. This paper introduces a relaxed version of Minimum Trace Factor Analysis (MTFA), a convex optimization method with roots dating back to the work of Ledermann in 1940. This relaxation is particularly effective at not overfitting to heteroskedastic perturbations and addresses the commonly cited Heywood cases in factor analysis and the recently identified "curse of ill-conditioning" for existing spectral methods. We provide theoretical guarantees on the accuracy of the resulting low rank subspace and the convergence rate of the proposed algorithm to compute that matrix. We develop a number of interesting connections to existing methods, including HeteroPCA, Lasso, and Soft-Impute, to fill an important gap in the already large literature on low rank matrix estimation. Numerical experiments benchmark our results against several recent proposals for dealing with heteroskedastic noise.

==> header/header.tex <==


% BASIC PACKAGES %

\usepackage{harvard}
\usepackage{graphicx}
\usepackage{enumerate}
\usepackage{url}
\usepackage{framed}
\usepackage{float}
\usepackage{comment}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{stackengine}
\usepackage{bm}

% MARGIN NOTES %

\usepackage{marginnote}
\usepackage{setspace}

\newcommand{\mnl}[1]{{\reversemarginpar \setstretch{0.64} %
	\marginnote{{\scriptsize \bluetext{\emph{#1}}}}} }

\newcommand{\mnr}[1]{{\normalmarginpar \setstretch{0.64} %
	\marginnote{{\scriptsize \bluetext{\emph{#1}}}}} }

\setlength\marginparwidth{64pt}

% ALGORITHMS %

\floatstyle{ruled}
%\newfloat{algorithm}{hpt}{lop}
%\floatname{algorithm}{Algorithm}


% TABLE PACKAGES %
\usepackage{booktabs}
\usepackage{xcolor}

% RAISE/LOWER %

\makeatletter
\newcommand{\raisemath}[1]{\mathpalette{\raisem@th{#1}}}
\newcommand{\raisem@th}[3]{\raisebox{#1}{$#2#3$}}
\makeatother

% HIDE MACRO %

\newif\ifhide
\hidetrue %\hidefalse
\newcommand{\hide}[1]{\ifhide {} \else {#1} \fi} 

% EMPHASIZE BOX %

\usepackage{empheq}
\newcommand{\widefbox}[1]{\fbox{\hspace{0.33in}#1\hspace{0.33in}}}



% ACCENTS %

\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}



% PROOFS %

\usepackage{amsthm}

\newtheoremstyle{mytheoremstyle}
{\topsep}                    % Space above
{\topsep}                    % Space below
{\itshape}                   % Body font
{}                           % Indent amount
{\bfseries}                  % Theorem head font
{.}                          % Punctuation after theorem head
{.5em}                       % Space after theorem head
{}  % Theorem head spec (can be left empty, meaning ‘normal’)

\theoremstyle{mytheoremstyle}
\newtheorem{thm}[theorem]{Theorem}

\newtheorem*{theo}{Theorem}
\newtheorem*{lemm}{Lemma}
\newtheorem*{defn}{Definition}
\newtheorem*{prop}{Proposition}
\newtheorem*{assm}{Assumption}
\newtheorem*{cond}{Condition}
\newtheorem*{remk}{Remark}
\newtheorem*{corr}{Corollary}


% REFERENCES & LABELS %

\usepackage{hyperref}
\hypersetup{colorlinks=true, allcolors=bamboo}


\newcommand{\ci}[1]{\citeasnoun{#1}}
\newcommand{\cic}[2]{\citeasnoun[#1]{#2}}

\newcommand{\hci}[2]{ \href{#2}{\ci{#1}} }
\newcommand{\hcic}[3]{ \href{#3}{\cic{#1}{#2}} }
\newcommand{\hcite}[2]{ \href{#2}{\cite{#1}} }

\newcommand{\req}[1]{(\ref{#1})}





